Deceptive Fairness Attacks on Graphs via Meta Learning

We study deceptive fairness attacks on graphs to answer the following question: How can we achieve poisoning attacks on a graph learning model to exacerbate the bias deceptively? We answer this question via a bi-level optimization problem and propose a meta learning-based framework named FATE. FATE is broadly applicable with respect to various fairness definitions and graph learning models, as well as arbitrary choices of manipulation operations. We further instantiate FATE to attack statistical parity and individual fairness on graph neural networks. We conduct extensive experimental evaluations on real-world datasets in the task of semi-supervised node classification. The experimental results demonstrate that FATE could amplify the bias of graph neural networks with or without fairness consideration while maintaining the utility on the downstream task. We hope this paper provides insights into the adversarial robustness of fair graph learning and can shed light on designing robust and fair graph learning in future studies.

==> 07acknowledgements.tex <==
\begin{acks}
\jian{to add after accepted}
\end{acks}

==> neurips_2023/00abstract.tex <==
\begin{abstract}
% Graph learning has demonstrated superb empirical performance in many real-world applications. Recent evidence has shown that graph learning techniques could be unfair in many scenarios, which motivates the study of algorithmic fairness on graphs. 
% % Despite the promising progress in 
% In fair graph learning, it is often assumed that the input graph is benevolent while its adversarial robustness remains under-explored, thus jeopardizing the reliability of fair graph learning. In this paper, we study fairness attacks on graph learning to answer the following question: \textit{How can we achieve poisoning attacks on a graph learning model to exacerbate the bias?} We answer this question via a bi-level optimization problem and propose a meta learning-based attacking framework named \method. The proposed framework is broadly applicable with respect to various fairness definitions and graph learning models, as well as arbitrary choices of manipulation operations. We further instantiate \method~to attack statistical parity on graph neural networks and conduct extensive experimental evaluations on real-world datasets in the task of semi-supervised node classification. The experimental results demonstrate that \method~could amplify the bias of graph neural networks with or without fairness consideration while achieving the best performance on the downstream task compared with all baseline methods. We hope this paper provides insights into the adversarial robustness of fair graph learning and can shed light on designing robust and fair graph learning in future studies.
We study fairness attacks on graph learning to answer the following question: \textit{How can we achieve poisoning attacks on a graph learning model to exacerbate the bias?} We answer this question via a bi-level optimization problem and propose a meta learning-based attacking framework named \method. The proposed framework is broadly applicable with respect to various fairness definitions and graph learning models, as well as arbitrary choices of manipulation operations. We further instantiate \method~to attack statistical parity and individual fairness on graph neural networks. We conduct extensive experimental evaluations on real-world datasets in the task of semi-supervised node classification. The experimental results demonstrate that \method~could amplify the bias of graph neural networks with or without fairness consideration while maintaining the utility on the downstream task. We hope this paper provides insights into the adversarial robustness of fair graph learning and can shed light on designing robust and fair graph learning in future studies.
\end{abstract}

==> neurips_2023/01introduction.tex <==
\vspace{-2mm}
\section{Introduction}
\vspace{-2mm}
% Graph learning plays a pivotal role in many real-world applications, including smart city~\cite{li2022domain}, community detection~\cite{wang2022ifig}, financial fraud detection~\cite{zhang2017hidden}, and drug discovery~\cite{liu2023molecular}. Important as it might be, evidence has shown that graph learning models could be unfair in high-stake applications. For example, COVID-19 vaccines are distributed in a way that is biased toward individuals with low income~\cite{rydland2022radically}. As a consequence, the unfair vaccine allocation not only puts these individuals at a higher risk of infection but also makes it harder to slow down virus propagation in the communities.

% As such, algorithmic fairness on graphs has received much research attention. It aims to ensure that a graph learning model would not perpetuate or amplify bias in the input graph, leading to discriminatory learning results. So far, fair graph learning techniques have been proposed to ensure various definitions of fairness, including group fairness~\cite{dai2021say}, individual fairness~\cite{kang2020inform}, and counterfactual fairness~\cite{ma2022learning}. %A common strategy to ensure fairness on graphs is to incorporate regularization related to fairness during model training in order to achieve a good balance between fairness and the model performance in the downstream task (e.g., accuracy in node classification or link prediction).

% Despite the substantial progress in ensuring fairness in graph learning, existing studies mostly assume the benevolence of input graphs while overlooking the fact that malicious activities in the real world are commonplace. For example, suppose that a graph-based news recommender system tries to recommend news that is neutral to the political interest of its users. A malicious user (e.g., an extremist) may create multiple profiles that show a strong preference for disinformation about one political party (i.e., the chosen party), and deliberately establish connections with users (i.e., the impacted users) who support another political party. Then the recommender system may only recommend negative information about the chosen party to the impacted users. As a consequence, this could potentially result in extremism and/or hate speech on the web. Thus, it is critical to ensure that the fair graph learning techniques are resilient to adversarial attacks on fairness, which we term as \textit{fairness attacks}.

% Evidence has shown that graph learning models are susceptible to adversarial attacks~\cite{dai2018adversarial, zugner2018adversarial, li2020adversarial}. Despite the substantial progress in attacking the graph learning models, existing studies mostly target to degrade the predictive accuracy of the graph learning models while overlooking the diverse intentions of malicious activities in the real world. 
Algorithmic fairness in graph learning has received much research attention~\cite{bose2019compositional, kang2020inform, kang2022rawlsgcn}. Despite its substantial progress, existing studies mostly assume the benevolence of input graphs and aim to ensure that the bias would not be perpetuated or amplified in the learning process. However, malicious activities in the real world are commonplace.
For example, consider a financial fraud detection system which utilizes a transaction network to classify whether a bank account is fraudulent or not~\cite{zhang2017hidden, wang2019semi}. An adversary may manipulate the transaction network (e.g., malicious banker with access to the transaction data, theft of bank accounts to make malicious transactions), so that the graph-based fraud detection model would exhibit unfair classification results with respect to people of different demographic groups. Consequently, a biased fraud detection model may infringe civil liberty to certain financial activities and impact the well-being of an individual negatively~\cite{cfpb2023cfpb}. It would also make the graph learning model fail to provide the same quality of service to people of certain demographic groups, causing the financial institutions to lose business in the communities of the corresponding demographic groups. Thus, it is critical to understand how resilient a graph learning model is with respect to adversarial attacks on fairness, which we term as \textit{fairness attacks}.

To date, fairness attack has not been well studied. Sporadic literature often follows two strategies: (1) adversarial data point injection, which is often designed for tabular data rather than graphs~\cite{solans2021poisoning, mehrabi2021exacerbating, chhabra2021fairness, van2022poisoning} or (2) adversarial edge injection, which only attacks the group fairness of a graph neural network~\cite{hussain2022adversarial}. It is thus crucial to study how to attack different fairness definitions for a variety of graph learning models.

To achieve this goal, we study the \underline{F}airness \underline{at}tacks on graph l\underline{e}arning (\method) problem. We formulate it as a bi-level optimization, where the lower-level problem optimizes a task-specific loss function to make the fairness attacks deceptive\textcolor{blue}{,} and the upper-level problem leverages the supervision signal to modify the input graph and maximize the bias function corresponding to a user-defined fairness definition. To solve the bi-level optimization problem, we propose a meta learning-based solver (\method), whose key idea is to compute the meta-gradient of the upper-level bias function with respect to the input graph to guide the fairness attacks. Compared with existing works, our proposed \method~framework has two major advantages. First, it is capable of attacking \textit{any} fairness definition on \textit{any} graph learning model, as long as the corresponding bias function and the task-specific loss function are differentiable. Second, it is equipped with the ability for either continuous or discretized poisoning attacks on the graph topology. We also briefly discuss its ability for poisoning attacks on node features in a later section.

%We further instantiate the bi-level optimization problem by attacking statistical parity, a commonly studied group fairness definition, on graph neural network (GNN). 

The major contributions of this paper are summarized as follows.
\begin{itemize}[
    align=left,
    leftmargin=1em,
    itemindent=0pt,
    labelsep=0pt,
    labelwidth=1em,
]
    \item \textbf{Problem definition.} We formally define the problem of fairness attacks on graph learning (the \method~problem). Based on the definition, we formulate it as a bi-level optimization problem, whose key idea is to maximize a bias function in the upper level while minimizing a task-specific loss function for a graph learning task \textcolor{blue}{in the lower level}.
    \item \textbf{Attacking framework.} We propose an end-to-end attacking framework named \method. It learns a perturbed graph topology via meta learning, such that the bias with respect to the learning results trained with the perturbed graph will be amplified.
    \item \textbf{Empirical evaluation.} We conduct experiments on three benchmark datasets to demonstrate the efficacy of our proposed \method~framework in amplifying the bias while being the most deceptive method (i.e., achieving the highest micro F1 score) on semi-supervised node classification.
\end{itemize}



==> neurips_2023/02preliminary.tex <==
\vspace{-2mm}
\section{Preliminaries and Problem Definition}
\vspace{-2mm}
% In this section, we first present the notation convention and key symbols used throughout the paper. Then we present a brief review for algorithmic fairness on graphs. Finally, we formally define the problem of fairness attacks on graphs.

% \begin{table}
% 	\centering
% 	\caption{Key symbols in the paper. \jian{maybe remove this table?}}
% 	\label{tab:symbols}
% 	\begin{tabular}{c|c}
% 		\hline 
% 		\textbf{Symbol} & \textbf{Description} \\
% 		\hline
% 		$\mathbf{A}$ & a matrix \\
% 		$\mathbf{A}^T$ & transpose of matrix ${\mathbf A}$ \\
% 		$\mathbf{x}$ & a vector \\
% 		\hline
% 		$\mathcal{G}$ & a graph \\
% 		$\mathcal{V}$ & a set of nodes \\
% 		$\mathbf{\widetilde A}$ & poisoned graph \\
% 		$\mathbf{X}$ & node feature matrix \\
% 		% $\mathbf{Y}^*$ & optimal learning results of the lower-level problem \\
% 		% $\mathbf{\widetilde Y}$ & optimal learning results on the poisoned graph \\
% 		$\Theta$ & a set of learnable variables \\
%             $\theta$ & a set of hyperparameters \\
% 		$l(\cdot)$ & task-specific loss function \\
% 		$b(\cdot)$ & bias function of a fairness definition \\
% 		\hline
% 	\end{tabular}
% \end{table}

\noindent \textbf{A -- Notations.} Throughout the paper, we use bold upper-case letter for matrix (e.g., $\mathbf{A}$), bold lower-case letter for vector (e.g., $\mathbf{x}$) and calligraphic letter for set (e.g., $\mathcal{G}$). We use superscript $^T$ to denote the transpose of a matrix/vector (e.g., $\mathbf{x}^T$ is the transpose of $\mathbf{x}$). Regarding matrix/vector indexing, we use conventions similar to NumPy in Python. For example, $\mathbf{A}\left[i, j\right]$ is the entry of $\mathbf{A}$ at the $i$-th row and $j$-th column; $\mathbf{x}\left[i\right]$ is the $i$-th entry of $\mathbf{x}$; $\mathbf{A}\left[i, :\right]$ and \textcolor{blue}{$\mathbf{A}\left[:, j\right]$} are the $i$-th row and $j$-th column of $\mathbf{A}$, respectively. %Table~\ref{tab:symbols} summarizes the key symbols used in this paper.

\noindent \textbf{B -- Algorithmic fairness.} The general principle of algorithmic fairness is to ensure the learning results would not favor one side or another.\footnote{\url{https://www.merriam-webster.com/dictionary/fairness}} Among several fairness definitions that follow this principle, group fairness~\cite{feldman2015certifying, hardt2016equality} and individual fairness~\cite{dwork2012fairness} are the most widely studied ones. Group fairness splits the entire population into multiple demographic groups by a sensitive attribute (e.g., gender) and ensure the parity of a statistical property among learning results of those groups. For example, statistical parity, a classic group fairness definition, guarantees the statistical independence between the learning results (e.g., predicted labels of a classification algorithm) and the sensitive attribute~\cite{feldman2015certifying}. Individual fairness suggests that similar individuals should be treated similarly. It is often formulated as a Lipschitz inequality such that distance between the learning results of two data points should be no larger than the difference between these two data points~\cite{dwork2012fairness}.

% Group fairness is one of the most intuitive fairness definitions. It often relies on a sensitive attribute (e.g., gender) to split the entire population into multiple demographic groups and ensure the parity among learning results of those groups. For example, statistical parity, which is one of the most fundamental group fairness definitions, aims to ensure an equal acceptance rate among different demographic groups. Mathematically, it is equivalent to the statistical independence between the learning results (e.g., predicted labels of a classification algorithm) and the sensitive attribute. Consider a classification problem with ${\hat y}$ being the predicted label, $s$ being the sensitive attribute whose attribute value is in the set $\mathcal{S}$. Statistical parity is defined as follows.
% \begin{equation}\label{eq:statistical_parity}
% 	\operatorname{P}\left[{\hat y} = 1\right] = \operatorname{P}\left[{\hat y} = 1|s = a\right],\quad \forall a\in\mathcal{S}
% \end{equation}

% Other than group fairness, individual fairness studies fairness in a finer-grained individual level. It asks for similar individuals to be treated similarly~\cite{dwork2012fairness}. Such principle is often formulated as a Lipschitz inequality $d_1\left(\mathbf{Y}[i, :], \mathbf{Y}[j, :]\right) \leq \epsilon d_2\left(i, j\right)$,
% \begin{equation}\label{eq:individual_fairness}
% 	d_1\left(\mathbf{Y}[i, :], \mathbf{Y}[j, :]\right) \leq \epsilon d_2\left(i, j\right)
% \end{equation}
% where $\mathbf{Y}$ is the learning results, $\epsilon$ is the Lipschitz constant, the left hand side $d_1\left(\mathbf{Y}[i, :], \mathbf{Y}[j, :]\right)$ measures the distance between the learning results $\mathbf{Y}[i, :]$ and $\mathbf{Y}[j, :]$ of data points $i$ and $j$, respectively, and $d_2\left(i, j\right)$ measures the distance between the two data points. Given a graph $\mathcal{G}=\{\mathbf{A}, \mathbf{X}\}$ with adjacency matrix $\mathbf{A}$ and node feature matrix $\mathbf{X}$, Kang et al.~\cite{kang2020inform} further define $d_1$ as the squared Frobenius distance and assume the existence of an oracle pairwise node similarity matrix $\mathbf{S}$. Then, the overall individual bias of $\mathcal{G}$ is further defined as $\operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$ where $\mathbf{L}_{\mathbf{S}}$ is the graph Laplacian of similarity matrix $\mathbf{S}$.

\noindent \textbf{C -- Problem definition.} Existing work~\cite{hussain2022adversarial} for fairness attacks on graphs randomly injects adversarial edges so that the disparity between the learning results of two different demographic groups would be amplified. However, it suffers from three major limitations. (1) First, it only attacks statistical parity while overlooking other fairness definitions (e.g., individual fairness~\cite{dwork2012fairness}). (2) Second, it only considers adversarial edge injection, excluding other manipulations like edge deletion or reweighting. Hence, it is essential to investigate the possibility to attack other fairness definitions on real-world graphs with an arbitrary choice of manipulation operations. (3) Third, it does not consider the utility of graph learning models while achieving the fairness attacks, resulting in performance degradation in the downstream tasks. However, an institution that applies the graph learning models are often utility-maximizing~\cite{liu2018delayed, baumann2022enforcing}. Thus, a performance degradation in the utility would make the fairness attacks not deceptive from the perspective of a utility-maximizing institution.

In this paper, we seek to overcome the aforementioned limitations. To be specific, given an input graph, an optimization-based graph learning model, and a user-defined fairness definition, we aim to learn a modified graph such that a bias function of the corresponding fairness definition would be maximized for \textit{effective} fairness attacks, while minimizing the task-specific loss function with respect to the graph learning model for \textit{deceptive} fairness attacks. Formally, we define the problem of fairness attacks on graph learning, which is referred to as the \method~problem.

\begin{problem}\label{prob:fate}
    \method: Fairness Attacks on Graph Learning
\end{problem}
\noindent \textbf{Given:} (1) An undirected graph $\mathcal{G}=\left\{\mathbf{A}, \mathbf{X}\right\}$; (2) a task-specific loss function $l(\mathcal{G}, \mathcal{Y}, \Theta, \theta)$ where $\mathcal{Y}$ is the graph learning results, $\Theta$ is the set of learnable variables and $\theta$ is the set of hyperparameters; (3) a bias function \textcolor{blue}{$b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)$} where $\Theta^*= \arg\min_{\Theta} l(\mathcal{G}, \mathcal{Y}, \Theta, \theta)$ and $\mathbf{F}$ is the matrix that contains auxiliary fairness-related information %for the corresponding fairness definition 
(e.g., sensitive attribute values of all nodes in $\mathcal{G}$ for group fairness, pairwise node similarity matrix for individual fairness); (4) an integer budget $B$.

\noindent \textbf{Find:} a poisoned graph $\mathcal{\widetilde G} = \left\{\mathbf{\widetilde A}, \mathbf{\widetilde X}\right\}$ which satisfies the following properties: (1) $d\left(\mathcal{G}, \mathcal{\widetilde G}\right) \leq B$ where $d\left(\mathcal{G}, \mathcal{\widetilde G}\right)$ is the distance between the input graph $\mathcal{G}$ and the poisoned graph $\mathcal{\widetilde G}$ (e.g., \textcolor{blue}{the entry-wise matrix norms $\left\|\mathbf{A} - \mathbf{\widetilde A}\right\|_{1,1} = \left\|\operatorname{vec}\left(\mathbf{A} - \mathbf{\widetilde A}\right)\right\|_1$, $\left\|\mathbf{X} - \mathbf{\widetilde X}\right\|_{1,1} = \left\|\operatorname{vec}\left(\mathbf{X} - \mathbf{\widetilde X}\right)\right\|_1$}); (2) the bias function $b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)$ is maximized for effectiveness; (3) the task-specific loss function $l\left(\mathcal{\widetilde G}, \mathcal{Y}, \Theta, \theta\right)$ is minimized for deceptiveness.


==> neurips_2023/03methodology.tex <==
\vspace{-2mm}
\section{Methodology}
\vspace{-2mm}
In this section, we first formulate Problem~\ref{prob:fate} as a bi-level optimization problem, followed by a generic meta learning-based solver named \method. %We instantiate Problem~\ref{prob:fate} to attack statistical parity on graph neural networks and present how to solve it with the proposed \method~framework. Finally, we discuss the generalization and variants of \method~in attacking other fairness definitions and graph learning models.

\vspace{-2mm}
\subsection{Problem Formulation}
\vspace{-2mm}
Given an input graph $\mathcal{G} = \left\{\mathbf{A}, \mathbf{X}\right\}$ with adjacency matrix $\mathbf{A}$ and node feature matrix $\mathbf{X}$, an attacker aims to learn a poisoned graph $\mathcal{\widetilde G}=\left\{\mathbf{\widetilde A}, \mathbf{\widetilde X}\right\}$ such that the graph learning model will be maximally biased when trained on $\mathcal{\widetilde G}$. In this work, we consider the following settings for the attacker.

\noindent \textbf{The goal of the attacker.} The attacker aims to amplify the bias of the graph learning results output by a victim graph learning model. And the bias to be amplified is a choice made by the attacker based on which fairness definition the attacker aims to attack.

\noindent \textbf{The knowledge of the attacker.} Following similar settings in \cite{hussain2022adversarial}, we assume the attacker has access to the adjacency matrix, the feature matrix of the input graph, and the sensitive attribute of all nodes in the graph. 
% \hh{do we have some justifications for these assumption, e.g., this somewhat represent the worst (?) case scanario because we assume attacker knows a lot of info of the gl model?}\jian{(1) For example, in supervised graph-based anomaly detection, the malicious banker may have access to all applicants' demographics (i.e., sensitive attribute) but only know a few node labels (i.e., anomaly or not) which is the ground-truth labels we use for training. (2) Besides, related work \cite{hussain2022adversarial} have the same assumption for sensitive attributes. (3) Empirically, I found that this provides the most stable performance in fairness attacks.} 
For a (semi-)supervised learning problem, we assume that the ground-truth labels of the training nodes are also available to the attacker. For example, for a graph-based financial fraud detection problem, the malicious banker may have access to the demographic information (i.e., sensitive attribute) of the account holders and also know whether some bank accounts are fraudulent or not, which are the ground-truth labels for training nodes. Similar to \cite{zugner2018adversarial, zugner2019adversarial, hussain2022adversarial}, the attacker has no knowledge about the parameters of the victim model. Instead, the attacker will perform a gray-box attack by attacking a surrogate graph learning model. 

\noindent \textbf{The capabilitiy of the attacker.} The attacker is able to perturb up to $B$ edges/features in the graph (i.e., \textcolor{blue}{the entry-wise matrix norms} $\left\|\mathbf{A} - \mathbf{\widetilde A}\right\|_{1,1} \leq B$ or $\left\|\mathbf{X} - \mathbf{\widetilde X}\right\|_{1,1} \leq B$).

Based on that, we formulate Problem~\ref{prob:fate} as a bi-level optimization problem as follows.
\begin{equation}\label{eq:bi-level}
\begin{aligned}
    \mathcal{\widetilde G} = 
    \arg&\max_{\mathcal{G}}\ b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)
    \quad
    \textrm{s.t.}\quad \Theta^* = \arg\min_{\Theta} l\left(\mathcal{G},\mathbf{Y}, \Theta, \theta\right),\ d\left(\mathcal{G}, \mathcal{\widetilde G}\right)\leq B 
\end{aligned}
\end{equation}
where the lower-level problem learns an optimal surrogate graph learning model $\Theta^*$ by minimizing $l\left(\mathcal{G},\mathbf{Y}, \Theta, \theta\right)$, the upper-level problem finds a poisoned graph $\mathcal{\widetilde G}$ that could maximize a bias function $b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)$ for the victim graph learning model and the distance between the input graph\textcolor{blue}{,} and the poisoned graph $d\left(\mathcal{G}, \mathcal{\widetilde G}\right)$ is constrained to satisfy the setting about the budgeted attack. Note that Eq.~\eqref{eq:bi-level} is applicable to attack \textit{any} fairness definition on \textit{any} graph learning model, as long as the bias function $b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)$ and the loss function $l\left(\mathcal{G},\mathbf{Y}, \Theta, \theta\right)$ are differentiable. % In the following, we briefly discuss a few examples.

\noindent \textbf{A -- Lower-level optimization problem.} A wide spectrum of graph learning models are essentially solving an optimization problem. 
% We briefly discuss three typical examples, including PageRank for ranking~\cite{page1999pagerank}, LINE (1st) for embedding~\cite{tang2015line} and graph convolutional network (GCN) for semi-supervised node classification~\cite{kipf2016semi}, and summarize them in Table~\ref{tab:graph_learning_examples}.
Take the graph convolutional network (GCN)~\cite{kipf2016semi} as an example. It learns the node representation by aggregating information from its neighborhood, i.e., message passing. Mathematically, for an $L$-layer GCN, the hidden representation at $k$-th layer can be represented as $\mathbf{E}^{(k)} = \sigma\left(\mathbf{\widehat A} \mathbf{E}^{(k-1)} \mathbf{W}^{(k)}\right)$ where $\sigma$ is a nonlinear activation function (e.g., ReLU), $\mathbf{\widehat A} = \mathbf{D}^{-1/2} \left(\mathbf{A} + \mathbf{I}\right) \mathbf{D}^{-1/2}$ with $\mathbf{D}$ being the degree matrix of $\left(\mathbf{A} + \mathbf{I}\right)$ and $\mathbf{W}^{(k)}$ is the learnable weight matrix of the $k$-th layer. Then the lower-level optimization problem aims to learn the set of parameters $\Theta^* = \{\mathbf{W}^{(k)} \vert k = 1, \ldots, L\}$ that could minimize a task-specific loss function (e.g., cross-entropy loss for semi-supervised node classification). For more examples of graph learning models from the optimization perspective, please refers to Appendix~\ref{sec:graph_learning_model_discussion}.
%For a victim GCN, its corresponding surrogate model could be a GCN with a different activation function $\sigma$, different hidden dimension, and different setting of learning rate during model training. A common choice of surrogate GCN is a linear GCN~\cite{zugner2018adversarial, zugner2019adversarial, hussain2022adversarial}. 

% \textit{Model \#1: PageRank.} It is a random walk-based ranking algorithm to measure node importance. Given a damping factor $c$ and a teleportation vector $\mathbf{e}$, it minimizes a smoothness term $c\left(\mathbf{r}^T \left(\mathbf{I} - \mathbf{A}\right) \mathbf{r}\right)$ and a query-specific term $\left(1-c\right)\|\mathbf{r} - \mathbf{e}\|$ to compute the ranking vector $\mathbf{r}$. For a victim PageRank, the attacker could attack a surrogate PageRank with different choices of damping factor $c$ and/or teleportation vector $\mathbf{e}$.

% \textit{Model \#2: LINE (1st).} It is a skip-gram-based node embedding model, it aims to map each node into a $h$-dimensional space such that the score $\mathbf{H}[j,:]\mathbf{H}[i,:]^T$ will be small for any two connected nodes $i$ and $j$. For a victim LINE (1st), the attacker could attack a surrogate LINE (1st) with different dimension $h$ in the embedding space and/or a different number of negative samples $g$

% \textit{Model \#3: Graph Convolutional Network.} It learns the node representation by aggregating information from its neighborhood, i.e., message passing. Mathematically, for an $L$-layer GCN, the hidden representation at $k$-th layer can be represented as $\mathbf{E}^{(k)} = \sigma\left(\mathbf{\widehat A} \mathbf{E}^{(k-1)} \mathbf{W}^{(k)}\right)$ where $\sigma$ is a nonlinear activation function (e.g., ReLU), $\mathbf{\widehat A} = \mathbf{D}^{-1/2} \left(\mathbf{A} + \mathbf{I}\right) \mathbf{D}^{-1/2}$ with $\mathbf{D}$ being the degree matrix of $\left(\mathbf{A} + \mathbf{I}\right)$ and $\mathbf{W}^{(k)}$ is the learnable weight matrix of at $k$-th layer. For a victim GCN, its corresponding surrogate model could be a GCN with a different activation function $\sigma$, different hidden dimension, and different setting of learning rate during model training. A common choice of surrogate GCN is a linear GCN~\cite{zugner2018adversarial, zugner2019adversarial, hussain2022adversarial}.

% \textit{Remarks.} Note that, for a nonparametric graph learning model (e.g., PageRank, LINE (1st)), we have $\Theta = \{\mathbf{Y}\}$ which is the set of learning results. For example, following Table~\ref{tab:graph_learning_examples}, we have $\Theta = \{\mathbf{r}\}$ for PageRank and $\Theta = \{\mathbf{H}\}$ for LINE (1st). For parametric graph learning models (e.g., GCN), $\Theta$ refers to the set of learnable weights, e.g., $\Theta = \{\mathbf{W}^{(1)}, \ldots, \mathbf{W}^{(L)}\}$ for an $L$-layer GCN.

\noindent \textbf{B -- Upper-level optimization problem.} To attack the fairness aspect of a graph learning model, we aim to maximize a differentiable bias function $b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)$ with respect to a user-defined fairness definition in the upper-level optimization problem. 
% In this work, we assume that the bias function is differentiable. 
% We briefly discuss choices of the bias function for group fairness and individual fairness. And we discuss choices of the bias function for two commonly used fairness definitions: (1) group fairness and (2) individual fairness.
For example, for statistical parity~\cite{feldman2015certifying}, the fairness-related auxiliary information matrix $\mathbf{F}$ can be defined as the one-hot demographic membership matrix, where $\mathbf{F}[i, j] = 1$ if and only if node $i$ belongs to $j$-th demographic group. Then the statistical parity is equivalent to the statistical independence between the learning results $\mathbf{Y}$ and $\mathbf{F}$. Based on that, existing studies propose several differentiable measurements of the statistical dependence between $\mathbf{Y}$ and $\mathbf{F}$ as the bias function. For example, Bose et al.~\cite{bose2019compositional} use mutual information $I(\mathbf{Y}; \mathbf{F}$) as the bias function; Prost et al.~\cite{prost2019toward} define the bias function as the Maximum Mean Discrepancy $\textit{MMD}\left(\mathcal{Y}_0, \mathcal{Y}_1\right)$ between the learning results of two different demographic groups $\mathcal{Y}_0$ and $\mathcal{Y}_1$.
% \textit{Group fairness.} We consider statistical parity~\cite{feldman2015certifying} here. The fairness-related auxiliary information matrix $\mathbf{F}$ can be defined as the one-hot demographic membership matrix, where $\mathbf{F}[i, j] = 1$ if and only if node $i$ belongs to $j$-th demographic group. Then the statistical parity is equivalent to the statistical independence between the learning results $\mathbf{Y}$ and $\mathbf{F}$. Based on that, existing studies propose several differentiable measurements of the statistical dependence between $\mathbf{Y}$ and $\mathbf{F}$ as the bias function. For example, Bose et al.~\cite{bose2019compositional} use mutual information $I(\mathbf{Y}; \mathbf{F}$) as the bias function; Prost et al.~\cite{prost2019toward} define the bias function as the Maximum Mean Discrepancy (MMD) $\textit{MMD}\left(\mathcal{Y}_0, \mathcal{Y}_1\right)$ between the learning results of two different demographic groups $\mathcal{Y}_0$ and $\mathcal{Y}_1$.
% For example, Prost et al.~\cite{prost2019toward} define the bias function as the Maximum Mean Discrepancy (MMD) between the learning results of two different demographic groups.
% \begin{equation}\label{eq:mmd}
% \begin{aligned}
%     \textit{MMD}\left(\mathcal{Y}_0, \mathcal{Y}_1\right) = 
%     & \frac{1}{n_0^2} \sum_{i, j = 1}^{n_0} k\left(\mathbf{Y}[i, :], \mathbf{Y}[j,:]\right) + \frac{1}{n_1^2} \sum_{i, j = 1}^{n_1} k\left(\mathbf{Y}[i, :], \mathbf{Y}[j,:]\right) \\
%     & - \frac{1}{n_0 n_1} \sum_{i = 1}^{n_0}\sum_{j = 1}^{n_1}k\left(\mathbf{Y}[i, :], \mathbf{Y}[j,:]\right) = b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)
% \end{aligned}
% \end{equation}
% where $k\left(\right)$ is the Gaussian kernel, $\mathcal{Y}_0 = \{\mathbf{Y}[i,:] \vert \forall S[i, 0] = 1\}$, $\mathcal{Y}_1 = \{\mathbf{Y}[i,:] \vert \forall S[i, 1] = 1\}$, $n_0 = \vert \mathcal{Y}_0 \vert$ is the cardinality of $\mathcal{Y}_0$ and $n_1 = \vert \mathcal{Y}_0 \vert$ is the cardinality of $\mathcal{Y}_1$. The intuition is that, if $\mathbf{Y}$ and $\mathbf{S}$ are independent, the distributions of $\mathcal{Y}_0$ and $\mathcal{Y}_1$ are the same, which refers to zero MMD between two distributions. Other than statistical parity, Eq.~\eqref{eq:mmd} can be applied to equal opportunity~\cite{hardt2016equality}, which asks for an equal true positive rate of two demographic groups, by replacing $\mathcal{Y}_0$ and $\mathcal{Y}_1$ to be the set of learning results whose corresponding nodes have ground-truth label equal to $1$ and belong to the demographic group $0$ and $1$, respectively.
 
% \textit{Individual fairness.} Building upon the principles in \cite{kang2020inform}, the fairness-related auxiliary information matrix $\mathbf{F}$ is defined as the oracle symmetric pairwise node similarity matrix $\mathbf{S}$ (i.e., $\mathbf{F} = \mathbf{S}$), where $\mathbf{S}[i,j]$ measures the similarity between node $i$ and node $j$. Kang et al.~\cite{kang2020inform} define that the overall individual bias to be $\operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$. Assuming that $\mathbf{Y}$ is the output of an optimization-based graph learning model, $\mathbf{Y}$ can be viewed as a function with respect to the input graph $\mathcal{G}$, which makes $\operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$ differentiable with respect to $\mathcal{G}$. Thus, the bias function $b(\cdot)$ can be naturally defined as the overall individual bias of the input graph $\mathcal{G}$, i.e., $b\left(\mathbf{Y}, \Theta^*, \mathbf{S}\right) = \operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$.

\vspace{-2mm}
\subsection{The \method~Framework}
\vspace{-2mm}
To solve Eq.~\eqref{eq:bi-level}, we propose a generic attacking framework named \method~to learn the poisoned graph. The key idea is to view Eq.~\eqref{eq:bi-level} as a meta learning problem, which aims to find suitable hyperparameter settings for a learning task~\cite{bengio2000gradient}, and treat the graph $\mathcal{G}$ as a hyperparameter. With that, we learn the poisoned graph $\mathcal{\widetilde G}$ using the meta-gradient of the bias function $b\left(\mathbf{Y}, \Theta^*, \mathbf{F}\right)$ with respect to $\mathcal{G}$. 
%The general workflow of our proposed \method~is as follows. First, we solve the lower-level optimization problem $\Theta^* = \arg\min_{\Theta} l\left(\mathcal{G},\mathbf{Y}, \Theta, \theta\right)$ and obtain the optimal solution $\Theta^*$. After that, we compute the meta-gradient of the bias function with respect to the graph $\mathcal{G}$ using the solution $\Theta^*$ obtained in the previous step. Finally, we poison the graph with the computed meta-gradient in a principled way for continuous/discretized attack. 
In the following, we introduce two key parts of \method~in details, including meta-gradient computation and graph poisoning with meta-gradient.

\noindent \textbf{A -- Meta-gradient computation.} %\hh{in gasoline, we call it hypergradient, and the overall method is iterative differentiation. do we need to clarify?}\jian{i think it should be fine. meta-gradient is more commonly used in meta-learning settings. for optimization, we use Eq 6 which is a first-order approximation of metagraient using only last pretraining step's parameter (used in maml and metattack as well).}
The key term to learn the poisoned graph is the meta-gradient of the bias function with respect to the graph $\mathcal{G}$. Before computing the meta-gradient, we assume that the lower-level optimization problem converges in $T$ epochs. Thus, we first pre-train the lower-level optimization problem by $T$ epochs to obtain the optimal model $\Theta^* = \Theta^{(T)}$ before computing the meta-gradient. The training of the lower-level optimization problem can also be viewed as a dynamic system with the following updating rule
\begin{equation}\label{eq:lower_level_dynamic}
    \Theta^{(t+1)} = \operatorname{opt}^{(t+1)}\left(\mathcal{G}, \Theta^{(t)}, \theta, \mathbf{Y}\right),~\forall t\in\{1, \ldots, T\}
\end{equation}
where $\Theta^{(1)}$ refers to $\Theta$ at initialization, $\operatorname{opt}^{(t+1)}(\cdot)$ is an optimizer that minimizes the lower-level loss function $l\left(\mathcal{G},\mathbf{Y}, \Theta^{(t)}, \theta\right)$ at $(t+1)$-th epoch. From the perspective of the dynamic system, by applying the chain rule and unrolling the training of lower-level problem with Eq.~\eqref{eq:lower_level_dynamic}, the meta-gradient $\nabla_{\mathcal{G}} b$ can be written as
\begin{equation}\label{eq:meta_grad_chain_rule}
    \nabla_{\mathcal{G}} b = \nabla_{\mathcal{G}} b\left(\mathbf{Y}, \Theta^{(T)}, \mathbf{F}\right) + \sum_{t=0}^{T-2} A_{t}B_{t+1} \dots B_{T-1}\nabla_{\theta^{(T)}} b\left(\mathbf{Y}, \Theta^{(T)}, \mathbf{F}\right)
\end{equation}
where $A_t=\nabla_{\mathcal{G}}\Theta^{(t+1)}$ and $B_t=\nabla_{\Theta^{(t)}}\Theta^{(t+1)}$. However, Eq.~\eqref{eq:meta_grad_chain_rule} is computationally expensive in both time and space. To further speed up the computation, we adopt a first-order approximation of the meta-gradient~\cite{finn2017model} and simplify the meta-gradient as 
\begin{equation}\label{eq:meta_grad_1st_order}
    \nabla_{\mathcal{G}} b \approx \nabla_{\Theta^{(T)}} b\left(\mathbf{Y}, \Theta^{(T)}, \mathbf{F}\right) \cdot \nabla_{\mathcal{G}} \Theta^{(T)}
\end{equation}
Since the input graph is undirected, the derivative of the symmetric adjacency matrix $\mathbf{A}$ can be computed as follows by applying the chain rule of a symmetric matrix~\cite{kang2019n2n}.
\begin{equation}\label{eq:grad_adj}
    \nabla_{\mathbf{A}} b \leftarrow \nabla_{\mathbf{A}} b + \left(\nabla_{\mathbf{A}} b\right)^T - \operatorname{diag}\left(\nabla_{\mathbf{A}} b\right)
\end{equation}
For the node feature matrix $\mathbf{X}$, its derivative is equal to the partial derivative $\nabla_{\mathbf{X}} b$ since it is often an asymmetric matrix.

\noindent \textbf{B -- Graph poisoning with meta-gradient.} After computing the meta-gradient of the bias function $\nabla_{\mathcal{G}} b$, we aim to poison the input graph guided by $\nabla_{\mathcal{G}} b$. We introduce two poisoning strategies: (1) continuous poisoning and (2) discretized poisoning. 

\noindent \textit{Continuous poisoning attack.} The continuous poisoning attack is straightforward by reweighting edges in the graph. We first compute the meta-gradient of the bias function $\nabla_{\mathbf{A}} b$, then use it to poison the input graph in a gradient descent-based updating rule as follows.
\begin{equation}\label{eq:poison_continuous}
    \mathbf{A} \leftarrow \mathbf{A} - \eta \nabla_{\mathbf{A}} b
\end{equation}
where $\eta$ is a learning rate to control the magnitude of the poisoning attack. The learning rate should satisfy $\eta \leq \frac{B}{\|\nabla_{\mathbf{A}}\|_{1,1}}$ to ensure that constraint on the budgeted attack.

\noindent \textit{Discretized poisoning attack.} The discretized poisoning attack aims to select a set of edges to be added/deleted. It is guided by a poisoning preference matrix defined as follows.
\begin{equation}\label{eq:modification_matrix}
    \nabla_{\mathbf{A}} = (\mathbf{1} - 2\mathbf{A}) \circ \nabla_\mathbf{A} b
\end{equation}
where $\mathbf{1}$ is an all-one matrix with the same dimension as $\mathbf{A}$ and $\circ$ denotes the Hadamard product. A large positive $\nabla_{\mathbf{A}}[i, j]$ indicates strong preference in adding an edge if nodes $i$ and $j$ are not connected (i.e., positive $\nabla_\mathbf{A} b [i, j]$, positive $(\mathbf{1} - 2\mathbf{A})[i, j]$) or deleting an edge if nodes $i$ and $j$ are connected (i.e., negative $\nabla_\mathbf{A} b [i, j]$, negative $(\mathbf{1} - 2\mathbf{A})[i, j]$). Then, a greedy selection strategy is applied to find the set of edges $\mathcal{E}_{\text{attack}}$ to be added/deleted.
\begin{equation}\label{eq:discretized_greedy}
    \mathcal{E}_{\text{attack}} = \operatorname{topk}(\nabla_{\mathbf{A}}, \delta)
\end{equation}
where $\operatorname{topk}(\nabla_{\mathbf{A}}, \delta)$ selects $\delta$ entries with highest preference score in $\nabla_{\mathbf{A}}$. Note that, if we only want to add edges without any deletion, all negative entries in $\nabla_\mathbf{A} b$ should be zeroed out before computing Eq.~\eqref{eq:modification_matrix}. Likewise, if edges are only expected to be deleted, all positive entries should be zeroed out. 

\noindent \textit{Remarks.} Poisoning node feature matrix $\mathbf{X}$ follows the same steps as poisoning adjacency matrix $\mathbf{A}$ without applying Eq.~\eqref{eq:grad_adj}.

\noindent \textbf{C -- Overall framework.} 
\method~generally works as follows. (1) We first pre-train the surrogate graph learning model and get the corresponding learning model $\Theta^{(T)}$ as well as the learning results $\mathbf{Y}^{(T)}$. (2) Then we compute the meta gradient of the bias function using Eqs.~\eqref{eq:meta_grad_1st_order} and \eqref{eq:grad_adj}. (3) Finally, we perform the discretized poisoning attack (Eqs.~\eqref{eq:modification_matrix} and \eqref{eq:discretized_greedy}) or continuous poisoning attack (Eq.~\eqref{eq:poison_continuous}). A detailed pseudo-code of \method~is provided in Appendix~\ref{sec:pseudocode}. %Note that \method~bears subtle differences with Metattack and \textsc{GaSoliNe} \hh{1. missing references for both. 2. will it be better to discuss this in the related work section?}\jian{i will move to related work.}, which also utilize meta learning for adversarial attacks and graph structure learning, respectively. (1) Metattack aims to degrade the utility of a graph neural network by maximizing the task-specific utility loss (e.g., cross entropy for node classification) in the upper-level optimization problem, whereas, in \method, the upper-level optimization problem maximizes a bias function rather than a task-specific utility loss. (2) \textsc{GaSoliNe} learns an optimal graph to boost the utility, whereas \method~is designed for a different purpose, i.e., attacking the fairness.
% Algorithm~\ref{alg:fate} summarizes the detailed steps on fairness attack with \method. To be specific, after initialization (lines 1 -- 3), we first pre-train the surrogate graph learning model (lines 6 -- 8) and get the corresponding learning model $\Theta^{(T)}$ and learning results $\mathbf{Y}^{(T)}$ (line 9). Then we compute the meta gradient of the bias function using Eqs.~\eqref{eq:meta_grad_1st_order} and \eqref{eq:grad_adj} (lines 10 -- 11) and perform the discretized poisoning attack (lines 12 -- 14) or continuous poisoning attack (lines 15 -- 17). Note that \method~bears subtle differences with Metattack and \textsc{GaSoliNe} \hh{1. missing references for both. 2. will it be better to discuss this in the related work section?}\jian{i will move to related work.}, which also utilize meta learning for adversarial attacks and graph structure learning, respectively. (1) Metattack aims to degrade the utility of a graph neural network by maximizing the task-specific utility loss (e.g., cross entropy for node classification) in the upper-level optimization problem, whereas, in \method, the upper-level optimization problem maximizes a bias function rather than a task-specific utility loss. (2) \textsc{GaSoliNe} learns an optimal graph to boost the utility, whereas \method~is designed for a different purpose, i.e., attacking the fairness.

\noindent \textbf{D -- Limitations.} 
Since \method~leverages the meta-gradient to poison the input graph, it requires the bias function $b\left(\mathbf{Y}, \Theta^{(T)}, \mathbf{F}\right)$ to be differentiable in order to calculate the meta-gradient $\nabla_{\mathcal{G}} b$. In Sections~\ref{sec:instantiation_group_fairness} and \ref{sec:instantiation_individual_fairness}, we present a carefully chosen bias function for \method. And we leave it for future work on exploring the ability of \method~in attacking other fairness definitions. Moreover, though the meta-gradient can be efficiently computed via auto-differentiation in many deep learning packages (e.g., PyTorch\footnote{\url{https://pytorch.org/}}, TensorFlow\footnote{\url{https://www.tensorflow.org/}}), it requires $O(n^2)$ space complexity to store the meta-gradient when attacking fairness via edge flipping. It is still a challenging open problem on how to efficiently compute the meta-gradient in terms of space. One possible remedy for discretized attack might be a low-rank approximation on the perturbation matrix formed by $\mathcal{E}_{\text{attack}}$. Since the difference between the benign graph and poisoned graph are often small and budgeted ($d\left(\mathcal{G}, \mathcal{\widetilde G}\right)\leq B$), it is likely that the edge manipulations may be around a few set of nodes, which makes the perturbation matrix to be an (approximately) low-rank matrix.


\vspace{-2mm}
\section{Instantiation \#1: Statistical Parity on Graph Neural Networks}\label{sec:instantiation_group_fairness}
\vspace{-2mm}
Here, we instantiate \method~framework by attacking statistical parity on graph neural networks in a binary node classification problem with a binary sensitive attribute. We briefly discuss how to choose (1) the surrogate graph learning model used by the attacker, (2) the task-specific loss function in the lower-level optimization problem and (3) the bias function in the upper-level optimization problem.
% In this section, we consider a binary node classification problem with a binary sensitive attribute and instantiate the proposed \method~framework by attacking statistical parity on graph neural networks. To instantiate \method, there are three key components, including the surrogate graph learning model used by the attacker, the task-specific loss function in the lower-level optimization problem, and the bias function in the upper-level optimization problem.

\noindent \textbf{A -- Surrogate graph learning model.} We assume that the surrogate model to be used by the attacker is a 2-layer linear GCN~\cite{wu2019simplifying} with different hidden dimensions and model parameters at initialization.

\noindent \textbf{B -- Lower-level loss function.} We consider a semi-supervised node classification task for the graph neural network to be attacked. Thus, the lower-level loss function is chosen as the cross entropy between the ground-truth label and the predicted label:
% \begin{equation}\label{eq:cross_entropy}
%     l\left(\mathcal{G},\mathbf{Y}, \Theta, \theta\right) = \frac{1}{\vert \mathcal{V}_{\text{train}} \vert} \sum_{i\in \mathcal{V}_{\text{train}}}\sum_{j=1}^{c} y_{i,j} \ln {\widehat y}_{i,j}
% \end{equation}
$l\left(\mathcal{G},\mathbf{Y}, \Theta, \theta\right) = \frac{1}{\vert \mathcal{V}_{\text{train}} \vert} \sum_{i\in \mathcal{V}_{\text{train}}}\sum_{j=1}^{c} y_{i,j} \ln {\widehat y}_{i,j}$, where $\mathcal{V}_{\text{train}}$ is the set of training nodes with ground-truth labels with $\vert \mathcal{V}_{\text{train}} \vert$ being its cardinality, $c$ is the number of classes, $y_{i,j}$ is a binary indicator of whether node $i$ belongs to class $j$ and ${\widehat y}_{i,j}$ is the prediction probability of node $i$ belonging to class $j$.

\noindent \textbf{C -- Upper-level bias function.} We aim to attack statistical parity in the upper-level problem, which asks for $\operatorname{P}\left[{\hat y} = 1\right] = \operatorname{P}\left[{\hat y} = 1|s = 1\right]$.
% \begin{equation}
%     \operatorname{P}\left[{\hat y} = 1\right] = \operatorname{P}\left[{\hat y} = 1|s = 1\right]
% \end{equation}
% Note that the downstream task is binary node classification. 
Suppose $p\left({\widehat y}\right)$ is the probability density function (PDF) of ${\widehat y}_{i, 1}$ for any node $i$ and $p\left({\widehat y} \vert s = 1\right)$ is the PDF of ${\widehat y}_{i, 1}$ for any node $i$ belong to the demographic group with sensitive attribute value $s = 1$. We observe that $\operatorname{P}\left[{\hat y} = 1\right]$ and $\operatorname{P}\left[{\hat y} = 1|s = 1\right]$ are equivalent to the cumulative distribution functions (CDF) of $p\left({\widehat y} < \frac{1}{2} \right)$ and $p\left({\widehat y} < \frac{1}{2} \vert s = 1\right)$ , respectively. To estimate both $\operatorname{P}\left[{\hat y} = 1\right]$ and $\operatorname{P}\left[{\hat y} = 1|s = 1\right]$ with a differentiable function, we first estimate their probability density functions ($p\left({\widehat y} < \frac{1}{2} \right)$ and $p\left({\widehat y} < \frac{1}{2} \vert s = 1\right)$) with kernel density estimation (KDE, Definition~\ref{defn:kde}).
\begin{defn}\label{defn:kde}
(Kernel density estimation~\cite{chen2017tutorial}) Given a set of $n$ IID samples $\{x_1, \ldots, x_n\}$ drawn from a distribution with an unknown probability density function $f$, the kernel density estimation of $f$ at point $\tau$ is defined as follows.
\begin{equation}\label{eq:kde}
    {\widetilde f}\left(\tau\right) = \frac{1}{na}\sum_{i=1}^{n} f_k\left(\frac{\tau - x_i}{a}\right)
\end{equation}
where ${\widetilde f}$ is the estimated probability density function, $f_k$ is the kernel function and $a$ is a non-negative bandwidth.
\end{defn}
Moreover, we assume the kernel function in KDE is the Gaussian kernel $f_k\left(x\right) = \frac{1}{\sqrt{2\pi}} e^{-x^2 / 2}$. %with the following form.
% \begin{equation}\label{eq:gaussian_kernel}
%     f_k\left(x\right) = \frac{1}{\sqrt{2\pi}} e^{-x^2 / 2}
% \end{equation}
% Even with the KDE-based PDF estimation, 
However, computing the CDF of a Gaussian distribution is non-trivial. Following~\cite{cho2020fair}, we leverage a tractable approximation of the Gaussian Q-function as follows.
\begin{equation}\label{eq:q_function}
    Q(\tau) = F_k\left(\tau\right) = \int_{\tau}^{\infty} f_k(x) dx \approx e^{-\alpha\tau^2 - \beta\tau - \gamma}
\end{equation}
where $f_k(x) = = \frac{1}{\sqrt{2\pi}} e^{-x^2 / 2}$ is a Gaussian distribution with zero mean, $\alpha=0.4920$, $\beta=0.2887$, $\gamma=1.1893$~\cite{lopez2011versatile}. The overall workflow of estimating $\operatorname{P}\left[{\hat y} = 1\right]$ is as follows.
\begin{itemize}[
    align=left,
    leftmargin=1em,
    itemindent=0pt,
    labelsep=0pt,
    labelwidth=1em,
]
    \item For any node $i$, get its prediction probability ${\widehat y}_{i, 1}$ with respect to class $1$;
    % \item [2.] Compute the mean probability overall nodes ${\bar y}_1 = \frac{1}{n}\sum_{i=1}^{n} {\widehat y}_{i, 1}$ where $n$ is number of nodes;
    \item Estimate the CDF $\operatorname{P}\left[{\hat y} = 1\right]$ using a Gaussian KDE with bandwidth $a$ by $\operatorname{P}\left[{\hat y} = 1\right] = \frac{1}{n}\sum_{i=1}^{n} \exp\left(-\alpha\left(\frac{0.5 - {\widehat y}_{i, 1}}{a}\right)^2 - \beta\left(\frac{0.5 - {\widehat y}_{i, 1}}{a}\right) - \gamma\right)$, 
    % \begin{equation}\label{eq:cdf_estimation}
    %     \operatorname{P}\left[{\hat y} = 1\right] = \frac{1}{n}\sum_{i=1}^{n} \exp\left(-\alpha\left(\frac{0.5 - {\widehat y}_{i, 1}}{a}\right)^2 - \beta\left(\frac{0.5 - {\widehat y}_{i, 1}}{a}\right) - \gamma\right)
    % \end{equation}
    where $\alpha=0.4920$, $\beta=0.2887$, $\gamma=1.1893$ and $\exp(x) = e^{x}$. %and $a$ is a non-negative bandwith for Gaussian KDE.
\end{itemize}
Note that $\operatorname{P}\left[{\hat y} = 1|s = 1\right]$ can be estimated with a similar procedure with minor modifications. The only modifications needed are: (1) get the prediction probability of nodes with $s=1$ and (2) compute the CDF using the Gaussian Q-function %Eq.~\eqref{eq:cdf_estimation} 
over nodes with $s=1$ rather than all nodes in the graph.

\vspace{-2mm}
\section{Instantiation \#2: Individual Fairness on Graph Neural Networks}\label{sec:instantiation_individual_fairness}
\vspace{-2mm}
We provide another instantiation of \method~framework by attacking individual fairness on graph neural networks. Here, we consider the same surrogate graph learning model (i.e., 2-layer linear GCN) and the same lower-level loss function (i.e., cross entropy) as described in Section~\ref{sec:instantiation_group_fairness}. To attack individual fairness, we define the upper-level bias function following the principles in \cite{kang2020inform}: the fairness-related auxiliary information matrix $\mathbf{F}$ is defined as the oracle symmetric pairwise node similarity matrix $\mathbf{S}$ (i.e., $\mathbf{F} = \mathbf{S}$), where $\mathbf{S}[i,j]$ measures the similarity between node $i$ and node $j$. Kang et al.~\cite{kang2020inform} define that the overall individual bias to be $\operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$. Assuming that $\mathbf{Y}$ is the output of an optimization-based graph learning model, $\mathbf{Y}$ can be viewed as a function with respect to the input graph $\mathcal{G}$, which makes $\operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$ differentiable with respect to $\mathcal{G}$. Thus, the bias function $b(\cdot)$ can be naturally defined as the overall individual bias of the input graph $\mathcal{G}$, i.e., $b\left(\mathbf{Y}, \Theta^*, \mathbf{S}\right) = \operatorname{Tr}\left(\mathbf{Y}^T \mathbf{L}_{\mathbf{S}} \mathbf{Y}\right)$.

==> neurips_2023/04experiments.tex <==
\section{Experiments}
\vspace{-2mm}

\subsection{Attacking Statistical Parity on Graph Neural Networks}\label{sec:result_group_fairness_gcn}
\vspace{-2mm}
\noindent \textbf{Settings.} We compare \method~with %4 
{\color{blue} 3} %\hh{but u list *3* baselines. check} 
baseline methods, i.e., Random, DICE~\cite{waniek2018hiding}, FA-GNN~\cite{hussain2022adversarial}, under the same setting as in Section~\ref{sec:instantiation_group_fairness}. That is, (1) the fairness definition to be attacked is statistical parity; (2) the downstream task is binary semi-supervised node classification with binary sensitive attributes. The experiments are conducted on 3 real-world datasets, i.e., Pokec-n, Pokec-z and Bail. Similar to existing works, we use the 50\%/25\%/25\% splits for train/validation/test sets. For all baseline methods, the victim models are set to GCN~\cite{kipf2016semi}. For each dataset, we use a fixed random seed to learn the poisoned graph corresponding to each baseline method. Then we train the victim model 5 times with different random seeds. For a fair comparison, we only attack the adjacency matrix in all experiments. Please refer to Appendix~\ref{sec:detailed_settings} for detailed experimental settings.

\begin{table*}
	\centering
	\caption{Effectiveness of attacking group fairness on GCN. \method~poisons the graph via both edge flipping (\method-flip) and edge addition (\method-add) while all other baselines poison the graph via edge addition. Higher is better ($\uparrow$) for micro F1 score (Micro F1) and $\spmetric$. Bold font indicates the success of fairness attack (i.e., $\spmetric$ is increased after fairness attack) with the highest micro F1 score. Underlined cell indicates the failure of fairness attack (i.e., $\spmetric$ is decreased after fairness attack).}
	\label{tab:results_group_fairness_gcn}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|cc|cc|cc|cc|cc}
		\hline
		\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Ptb.}} & \multicolumn{2}{c|}{\textbf{Random}} & \multicolumn{2}{c|}{\textbf{DICE}} & \multicolumn{2}{c|}{\textbf{FA-GNN}} & \multicolumn{2}{c|}{\textbf{\method-flip}} & \multicolumn{2}{c}{\textbf{\method-add}}\\
		\cline{3-12}
		& & \textbf{Micro F1 ($\uparrow$)} & \textbf{$\spmetric$ ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{$\spmetric$ ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{$\spmetric$ ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{$\spmetric$ ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{$\spmetric$ ($\uparrow$)} \\
            \hline
		\multirow{6}{*}{\textbf{Pokec-n}} & $0.00$ & $67.5 \pm 0.3$ & $7.1 \pm 0.4$ & $67.5 \pm 0.3$ & $7.1 \pm 0.4$ & $67.5 \pm 0.3$ & $7.1 \pm 0.4$ & $67.5 \pm 0.3$ & $7.1 \pm 0.4$ & $67.5 \pm 0.3$ & $7.1 \pm 0.4$ \\
										  & $0.05$ & \underline{$68.0 \pm 0.3$} & \underline{$6.2 \pm 0.8$} & \underline{$67.6 \pm 0.2$} & \underline{$6.8 \pm 0.3$} & \underline{$67.8 \pm 0.1$} & \underline{$3.3 \pm 0.4$} & $\bf 67.9 \pm 0.4$ & $\bf 9.3 \pm 1.2$ & $\bf 67.9 \pm 0.4$ & $\bf 9.3 \pm 1.2$ \\
										  & $0.10$ & $66.8 \pm 0.8$ & $7.3 \pm 0.7$ & \underline{$66.1 \pm 0.5$} & \underline{$6.6 \pm 1.1$} & $66.0 \pm 0.2$ & $11.5 \pm 0.6$ & $\bf 68.2 \pm 0.6$ & $\bf 9.8 \pm 1.5$ & $\bf 68.2 \pm 0.6$ & $\bf 9.8 \pm 1.5$ \\
										  & $0.15$ & $66.7 \pm 0.4$ & $8.1 \pm 0.4$ & $65.6 \pm 0.4$ & $7.7 \pm 0.8$ & $66.0 \pm 0.4$ & $15.6 \pm 3.0$ & $\bf 68.0 \pm 0.3$ & $\bf 11.5 \pm 1.0$ & $\bf 68.0 \pm 0.3$ & $\bf 11.5 \pm 1.0$ \\
										  & $0.20$ & $66.3 \pm 0.7$ & $8.6 \pm 1.8$ & \underline{$64.2 \pm 0.4$} & \underline{$3.4 \pm 0.9$} & $65.8 \pm 0.1$ & $18.4 \pm 0.7$ & $\bf 68.2 \pm 0.5$ & $\bf 12.0 \pm 1.8$ & $\bf 68.2 \pm 0.5$ & $\bf 12.0 \pm 1.8$ \\
										  & $0.25$ & $66.2 \pm 0.6$ & $8.5 \pm 0.8$ & \underline{$63.4 \pm 0.2$} & \underline{$6.3 \pm 0.8$} & $66.6 \pm 0.2$ & $23.3 \pm 0.5$ & $\bf 68.3 \pm 0.4$ & $\bf 12.1 \pm 2.1$ & $\bf 68.3 \pm 0.4$ & $\bf 12.1 \pm 2.1$ \\
		\hline
		\multirow{6}{*}{\textbf{Pokec-z}} & $0.00$ & $68.4 \pm 0.4$ & $6.6 \pm 0.9$ & $68.4 \pm 0.4$ & $6.6 \pm 0.9$ & $68.4 \pm 0.4$ & $6.6 \pm 0.9$ & $68.4 \pm 0.4$ & $6.6 \pm 0.9$ & $68.4 \pm 0.4$ & $6.6 \pm 0.9$ \\
										  & $0.05$ & \underline{$68.8 \pm 0.4$} & \underline{$6.4 \pm 0.6$} & $67.4 \pm 0.5$ & $6.6 \pm 0.3$ & \underline{$68.1 \pm 0.3$} & \underline{$2.2 \pm 0.4$} & $\bf 68.7 \pm 0.4$ & $\bf 6.7 \pm 1.4$ & $\bf 68.7 \pm 0.4$ & $\bf 6.7 \pm 1.4$ \\
										  & $0.10$ & $\bf 68.7 \pm 0.3$ & $\bf 8.0 \pm 0.6$ & \underline{$66.5 \pm 0.2$} & \underline{$6.3 \pm 0.8$} & $67.7 \pm 0.4$ & $13.5 \pm 0.9$ & $\bf 68.7 \pm 0.6$ & $\bf 7.5 \pm 0.7$ & $\bf 68.7 \pm 0.6$ & $\bf 7.5 \pm 0.7$ \\
										  & $0.15$ & $67.9 \pm 0.3$ & $9.1 \pm 0.8$ & \underline{$65.9 \pm 0.8$} & \underline{$5.5 \pm 1.3$} & $66.6 \pm 0.4$ & $16.9 \pm 2.6$ & $\bf 69.0 \pm 0.8$ & $\bf 8.5 \pm 1.1$ & $\bf 69.0 \pm 0.8$ & $\bf 8.5 \pm 1.1$ \\
										  & $0.20$ & $\bf 68.5 \pm 0.4$ & $\bf 9.3 \pm 1.0$ & $62.9 \pm 0.7$ & $8.7 \pm 1.0$ & $66.1 \pm 0.2$ & $25.4 \pm 1.3$ & $\bf 68.5 \pm 0.6$ & $\bf 8.8 \pm 1.1$ & $\bf 68.5 \pm 0.6$ & $\bf 8.8 \pm 1.1$ \\
										  & $0.25$ & $68.3 \pm 0.5$ & $7.3 \pm 0.5$ & \underline{$63.9 \pm 0.4$} & \underline{$6.0 \pm 1.0$} & $65.5 \pm 0.6$ & $22.3 \pm 2.8$ & $\bf 68.5 \pm 1.1$ & $\bf 8.6 \pm 2.5$ & $\bf 68.5 \pm 1.1$ & $\bf 8.6 \pm 2.5$\\
		
		\hline
		\multirow{6}{*}{\textbf{Bail}} & $0.00$ & $93.1 \pm 0.2$ & $8.0 \pm 0.2$ & $93.1 \pm 0.2$ & $8.0 \pm 0.2$ & $93.1 \pm 0.2$ & $8.0 \pm 0.2$ & $93.1 \pm 0.2$ & $8.0 \pm 0.2$ & $93.1 \pm 0.2$ & $8.0 \pm 0.2$ \\
									   & $0.05$ & $\bf 92.7 \pm 0.2$ & $\bf 8.1 \pm 0.0$ & $91.6 \pm 0.2$ & $8.5 \pm 0.1$ & $91.7 \pm 0.1$ & $10.0 \pm 0.4$ & $92.6 \pm 0.1$ & $8.6 \pm 0.1$ & $92.5 \pm 0.1$ & $8.6 \pm 0.1$ \\
									   & $0.10$ & \underline{$92.2 \pm 0.2$} & \underline{$7.8 \pm 0.2$} & $90.3 \pm 0.1$ & $8.5 \pm 0.1$ & $90.5 \pm 0.0$ & $10.3 \pm 0.4$ & $\bf 92.4 \pm 0.1$ & $\bf 8.9 \pm 0.1$ & $\bf 92.4 \pm 0.1$ & $\bf 8.6 \pm 0.1$  \\
									   & $0.15$ & \underline{$91.9 \pm 0.2$} & \underline{$7.8 \pm 0.1$} & \underline{$89.2 \pm 0.1$} & \underline{$7.7 \pm 0.1$} & $90.0 \pm 0.2$ & $8.4 \pm 0.2$ & $92.2 \pm 0.2$ & $9.1 \pm 0.1$ & $\bf 92.3 \pm 0.1$ & $\bf 9.1 \pm 0.1$ \\
									   & $0.20$ & \underline{$91.6 \pm 0.2$} & \underline{$7.8 \pm 0.1$} & $88.3 \pm 0.1$ & $8.3 \pm 0.1$ & \underline{$89.7 \pm 0.1$} & \underline{$7.4 \pm 0.4$} & $92.2 \pm 0.2$ & $9.3 \pm 0.1$ & $\bf 92.3 \pm 0.1$ & $\bf 9.3 \pm 0.2$ \\
									   & $0.25$ & $91.4 \pm 0.1$ & $8.3 \pm 0.1$ & \underline{$87.8 \pm 0.0$} & \underline{$7.8 \pm 0.1$} & \underline{$89.8 \pm 0.2$} & \underline{$5.2 \pm 0.2$} & $\bf 92.1 \pm 0.1$ & $\bf 9.1 \pm 0.2$ & $\bf 92.1 \pm 0.1$ & $\bf 9.1 \pm 0.3$ \\
		\hline
	\end{tabular}
	}
 \vspace{-7mm}
\end{table*}

\noindent \textbf{Main results.} For \method, we conduct fairness attacks via both edge flipping (\method-flip in {\color{blue} Table~\ref{tab:results_group_fairness_gcn}}
% Table~\ref{tab:results_gcn} \hh{Table 5 is not in the main body. check}) 
and edge addition (\method-add in Table~\ref{tab:results_group_fairness_gcn}). For all other baseline methods, edges are only added. The effectiveness of fairness attacks on GCN are presented in {\color{blue} Table~\ref{tab:results_group_fairness_gcn}}.
% Tables~\ref{tab:results_gcn} \hh{Table 5 is not in the main body. check}. 
From {\color{blue} the table}, we have the following key observations: (1) \method-flip and \method-add are the only methods that consistently succeed in fairness attacks, while all other baseline methods might fail in some cases (indicated by the underlined $\spmetric$) because of the decrease in $\spmetric$. (2) \method-flip and \method-add can not only amplify $\spmetric$ consistently, but also achieve the best micro F1 score on node classification, which makes \method-flip and \method-add more deceptive than all baseline methods. Notably, \method-flip and \method-add are able to even increase micro F1 score on all datasets, while other baseline methods attack the graph neural networks at the expense of utility (micro F1 score). (3) Though FA-GNN could make the model more biased in some cases, it cannot guarantee consistent success in fairness attacks on all three datasets as shown by the underlined $\spmetric$ in both tables. All in all, our proposed \method~framework %is the framework that 
consistently succeeds in fairness attacks while being the most deceptive (i.e., highest micro F1 score).

\noindent \textbf{Effect of the perturbation rate.} 
From Table~\ref{tab:results_group_fairness_gcn}, we have the following observations. First, $\spmetric$ tends to increase when the perturbation rate increases, which demonstrates the effectiveness of \method-flip and \method-add for attacking fairness. Though in some cases $\spmetric$ might have a marginal decrease, \method-flip and \method-add still successfully attack the fairness compared with GCN trained on the benign graph by being larger to the $\spmetric$ when perturbation rate (Ptb.) is 0. Second, \method-flip and \method-add are deceptive, meaning that the micro F1 scores is close to or even higher than the micro F1 scores on the benign graph compared with the corresponding metrics trained {\color{blue} on the poisoned graphs}. In summary, across different perturbation rates, \method-flip and \method-add are both effective, i.e., amplifying more bias with higher perturbation rate, and deceptive, i.e., achieving similar or even higher micro F1 score.

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=.98\textwidth]{figs/group_fairness_label_sensitive_label_analysis.png}
    \vspace{-2mm}
    \caption{}
    \label{fig:group_fairness_label_sensitive_label_analysis}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=.98\textwidth]{figs/group_fairness_same_label_value_analysis.png}
    \vspace{-2mm}
    \caption{}    
    \label{fig:group_fairness_same_label_value_analysis}
\end{subfigure}
\vspace{-2mm}
\caption{Attacking statistical parity with \method-flip. (a) Ratios of flipped edges that connect two nodes with same/different label or sensitive attribute (sens. attr.). (b) SL (abbreviation for same label) refers to the ratios of flipped edges whose two endpoints are both from the same class. SSA (abbreviation for same sensitive attribute) refers to the ratios of manipulated edges whose two endpoints are both from the same demographic group. Majority/minority classes are determined by splitting the training nodes based on their class labels. The protected group is the demographic group with fewer nodes.}
\label{fig:analysis_group_fairness_gcn}
\vspace{-6mm}
\end{figure}
\noindent \textbf{Analysis on the manipulated edges.} Here, we aim to characterize the properties of edges that are flipped by \method~(i.e., \method-flip) in attacking statistical parity. The reason to only analyze \method-flip is that the majority of edges manipulated by \method-flip on all three datasets is by addition (i.e., flipping from non-existing to existing). Figure~\ref{fig:group_fairness_same_label_value_analysis} suggests that, if the two endpoints of a manipulated edge share the same class label or same sensitive attribute value, these two endpoints are most likely from the minority class and protected group. Combining Figures~\ref{fig:group_fairness_label_sensitive_label_analysis} and \ref{fig:group_fairness_same_label_value_analysis}, \method~would significantly increase the number of edges that are incident to nodes in the minority class and/or protected group. 


\noindent \textbf{More experimental results.} Due to the space limitation, we defer more experimental results on attacking statistical parity on graph neural networks in Appendix~\ref{sec:additional_results_group_fairness}. More specifically, we present the performance evaluation under different metrics, i.e., Macro F1 and AUC, as well as the effectiveness of \method~with a different victim model, i.e., FairGNN~\cite{dai2021say}, which ensures statistical parity.



\vspace{-2mm}
\subsection{Attacking Individual Fairness on Graph Neural Networks}\label{sec:result_individual_fairness_gcn}
\vspace{-2mm}
\noindent \textbf{Settings.} To showcase the ability of \method~on attacking the individual fairness (Section~\ref{sec:instantiation_individual_fairness}), we further compare \method~with the same set of baseline methods (Random, DICE~\cite{waniek2018hiding}, FA-GNN~\cite{hussain2022adversarial}) on the same set of datasets (Pokec-n, Pokec-z, Bail). We follow the settings as in Section~\ref{sec:instantiation_individual_fairness}. We use the 50\%/25\%/25\% splits for train/validation/test sets with GCN~\cite{kipf2016semi} being the victim model. For each dataset, we use a fixed random seed to learn the poisoned graph corresponding to each baseline method. Then we train the victim model 5 times with different random seeds. And each entry in the oracle pairwise node similarity matrix is computed by the cosine similarity of the corresponding rows in the adjacency matrix. That is, $\mathbf{S}[i, j] = \operatorname{cos}\left(\mathbf{A}[i, :], A[j, :]\right)$, where $\operatorname{cos}\left(\right)$ is the function to compute cosine similarity. For a fair comparison, we only attack the adjacency matrix in all experiments. Please refer to Appendix~\ref{sec:detailed_settings} for detailed experimental settings.




\noindent \textbf{Main results.} We test \method~with both edge flipping (\method-flip in Table~\ref{tab:results_individual_fairness_gcn}) and edge addition (\method-add in Table~\ref{tab:results_individual_fairness_gcn}), while all other baseline methods only add edges. From Table~\ref{tab:results_individual_fairness_gcn}, we have two key observations. (1) \method-flip and \method-add are effective: they are the only methods that could consistently attack individual fairness whereas all other baseline methods mostly fail to attack individual fairness. (2) \method-flip and \method-add are deceptive: they achieve comparable or even better utility on all datasets compared with the utility on the benign graph. Hence, \method~framework is able to achieve effective and deceptive attacks to exacerbate individual bias.


\noindent \textbf{Effect of the perturbation rate.} From Table~\ref{tab:results_individual_fairness_gcn}, we obtain similar observations as in Section~\ref{sec:result_group_fairness_gcn} for Bail dataset. While for Pokec-n and Pokec-z, the correlation between the perturbation rate (Ptb.) and the individual bias is weaker. One possible reason is that: for Pokec-n and Pokec-z, the discrepancy between the oracle pairwise node similarity matrix and the benign graph is larger. Since the individual bias is computed using the oracle pairwise node similarity matrix rather than the benign/poisoned adjacency matrix, a higher perturbation rate to poison the adjacency matrix may have less impact on the computation of individual bias.

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=.98\textwidth]{figs/individual_fairness_label_sensitive_label_analysis.png}
    \vspace{-2mm}
    \caption{}
    \label{fig:individual_fairness_label_sensitive_label_analysis}
\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=.98\textwidth]{figs/individual_fairness_same_label_value_analysis.png}
    \vspace{-2mm}
    \caption{}
    \label{fig:individual_fairness_same_label_value_analysis}
\end{subfigure}
\vspace{-2mm}
\caption{Attacking individual fairness with \method-flip. (a) Ratios of flipped edges that connect two nodes with same/different label. (b) Ratios of flipped edges whose two endpoints are both from the majority/minority class. Majority/minority classes are formed by splitting the training nodes based on their class labels.}
\label{fig:analysis_individual_fairness_gcn}
\vspace{-4mm}
\end{figure}

\noindent \textbf{Analysis on the manipulated edges.} Since the majority of edges manipulated by \method-flip is through addition, we only analyze \method-flip here. From Figure~\ref{fig:analysis_individual_fairness_gcn}, we can find out that \method~tends to manipulate edges from the same class (especially from the minority class). In this way, \method~would find edges that could increase individual bias and improve the utility of the minority class in order to make the fairness attack deceptive.



\begin{table*}
	\centering
	\caption{Effectiveness of attacking individual fairness on GCN. \method~poisons the graph via both edge flipping (\method-flip) and edge addition (\method-add) while all other baselines poison the graph via edge addition. Higher is better ($\uparrow$) for micro F1 score (Micro F1) and InFoRM bias (Bias). Bold font indicates the success of fairness attack (i.e., bias is increased after attack) with the highest micro F1 score. Underlined cell indicates the failure of fairness attack (i.e., $\spmetric$ is decreased after attack).}
	\label{tab:results_individual_fairness_gcn}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|cc|cc|cc|cc|cc}
		\hline
		\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Ptb.}} & \multicolumn{2}{c|}{\textbf{Random}} & \multicolumn{2}{c|}{\textbf{DICE}} & \multicolumn{2}{c|}{\textbf{FA-GNN}} & \multicolumn{2}{c|}{\textbf{\method-flip}} & \multicolumn{2}{c}{\textbf{\method-add}}\\
		\cline{3-12}
		& & \textbf{Micro F1 ($\uparrow$)} & \textbf{Bias ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{Bias ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{Bias ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{Bias ($\uparrow$)} & \textbf{Micro F1 ($\uparrow$)} & \textbf{Bias ($\uparrow$)} \\
            \hline
		\multirow{6}{*}{\textbf{Pokec-n}} & $0.00$ & $67.5 \pm 0.3$ & $0.9 \pm 0.2$ & $67.5 \pm 0.3$ & $0.9 \pm 0.2$ & $67.5 \pm 0.3$ & $0.9 \pm 0.2$ & $67.5 \pm 0.3$ & $0.9 \pm 0.2$ & $67.5 \pm 0.3$ & $0.9 \pm 0.2$ \\
										  & $0.05$ & $67.6 \pm 0.3$ & $1.6 \pm 0.3$ & $66.9 \pm 0.3$ & $1.6 \pm 0.2$ & $\bf 67.8 \pm 0.5$ & $\bf 1.9 \pm 0.2$ & $\bf 67.8 \pm 0.3$ & $\bf 1.2 \pm 0.4$ & $67.6 \pm 0.3$ & $1.5 \pm 0.6$ \\
										  & $0.10$ & $67.2 \pm 0.5$ & $1.4 \pm 0.3$ & $65.3 \pm 0.7$ & $1.1 \pm 0.1$ & $67.4 \pm 0.4$ & $1.2 \pm 0.2$ & $\bf 67.9 \pm 0.4$ & $\bf 1.3 \pm 0.3$ & $67.7 \pm 0.4$ & $1.6 \pm 0.4$ \\
										  & $0.15$ & $67.2 \pm 0.3$ & $1.2 \pm 0.4$ & $63.9 \pm 0.6$ & $1.1 \pm 0.2$ & $66.1 \pm 0.3$ & $1.5 \pm 0.3$ & $\bf 67.8 \pm 0.4$ & $\bf 1.2 \pm 0.2$ & $67.6 \pm 0.2$ & $1.1 \pm 0.3$ \\
										  & $0.20$ & $66.6 \pm 0.3$ & $1.1 \pm 0.2$ & \underline{$63.8 \pm 0.1$} & \underline{$0.8 \pm 0.1$} & $65.7 \pm 0.6$ & $1.5 \pm 0.3$ & $67.3 \pm 0.4$ & $1.1 \pm 0.3$ & $\bf 68.2 \pm 1.0$ & $\bf 1.7 \pm 0.8$ \\
										  & $0.25$ & $66.7 \pm 0.3$ & $1.3 \pm 0.4$ & \underline{$62.5 \pm 0.4$} & \underline{$0.6 \pm 0.0$} & $65.2 \pm 0.5$ & $1.3 \pm 0.4$ & $\bf 67.8 \pm 0.8$ & $\bf 1.4 \pm 0.7$ & $\bf 67.9 \pm 0.9$ & $\bf 1.4 \pm 0.7$ \\
		\hline
		\multirow{6}{*}{\textbf{Pokec-z}} & $0.00$ & $68.4 \pm 0.4$ & $2.6 \pm 0.7$ & $68.4 \pm 0.4$ & $2.6 \pm 0.7$ & $68.4 \pm 0.4$ & $2.6 \pm 0.7$ & $68.4 \pm 0.4$ & $2.6 \pm 0.7$ & $68.4 \pm 0.4$ & $2.6 \pm 0.7$ \\
										  & $0.05$ & $\bf 69.0 \pm 0.4$ & $\bf 3.4 \pm 0.5$ & $67.1 \pm 0.5$ & $2.7 \pm 1.0$ & $68.1 \pm 0.4$ & $2.9 \pm 0.3$ & $68.7 \pm 0.5$ & $2.9 \pm 0.5$ & $68.7 \pm 0.4$ & $3.1 \pm 1.0$ \\
										  & $0.10$ & \underline{$68.7 \pm 0.1$} & \underline{$2.4 \pm 0.5$} & \underline{$66.3 \pm 0.6$} & \underline{$1.7 \pm 0.6$} & \underline{$68.2 \pm 0.5$} & \underline{$1.7 \pm 0.5$} & $\bf 69.0 \pm 0.6$ & $\bf 2.9 \pm 0.6$ & $\bf 69.0 \pm 0.5$ & $\bf 3.0 \pm 0.6$ \\
										  & $0.15$ & $67.9 \pm 0.3$ & $2.8 \pm 0.3$ & \underline{$65.5 \pm 0.3$} & \underline{$1.4 \pm 0.3$} & \underline{$67.0 \pm 0.5$} & \underline{$1.3 \pm 0.2$} & $68.6 \pm 0.5$ & $2.9 \pm 0.6$ & $\bf 69.0 \pm 0.7$ & $\bf 2.7 \pm 0.4$ \\
										  & $0.20$ & \underline{$67.9 \pm 0.3$} & \underline{$2.2 \pm 0.6$} & \underline{$64.2 \pm 0.4$} & \underline{$0.7 \pm 0.3$} & \underline{$66.1 \pm 0.1$} & \underline{$1.6 \pm 0.5$} & $68.8 \pm 0.4$ & $3.0 \pm 0.4$ & $\bf 69.2 \pm 0.4$ & $\bf 2.9 \pm 0.3$ \\
										  & $0.25$ & \underline{$67.6 \pm 0.3$} & \underline{$1.9 \pm 0.3$} & \underline{$64.2 \pm 0.3$} & \underline{$0.5 \pm 0.1$} & \underline{$65.1 \pm 0.3$} & \underline{$1.9 \pm 0.6$} & $69.1 \pm 0.3$ & $2.9 \pm 0.7$ & $\bf 69.3 \pm 0.3$ & $\bf 2.7 \pm 0.6$\\
		
		\hline
		\multirow{6}{*}{\textbf{Bail}} & $0.00$ & $93.1 \pm 0.2$ & $7.2 \pm 0.6$ & $93.1 \pm 0.2$ & $7.2 \pm 0.6$ & $93.1 \pm 0.2$ & $7.2 \pm 0.6$ & $93.1 \pm 0.2$ & $7.2 \pm 0.6$ & $93.1 \pm 0.2$ & $7.2 \pm 0.6$ \\
									   & $0.05$ & $92.1 \pm 0.3$ & $8.0 \pm 1.9$ & \underline{$91.8 \pm 0.1$} & \underline{$7.1 \pm 1.1$} & \underline{$91.2 \pm 0.2$} & \underline{$5.6 \pm 0.7$} & $\bf 93.0 \pm 0.3$ & $7.8 \pm 1.0$ & $92.9 \pm 0.2$ & $7.7 \pm 1.0$ \\
									   & $0.10$ & $91.6 \pm 0.1$ & $7.3 \pm 1.2$ & \underline{$90.3 \pm 0.1$} & \underline{$6.1 \pm 0.6$} & \underline{$90.3 \pm 0.1$} & \underline{$5.1 \pm 0.4$} & $\bf 93.0 \pm 0.1$ & $\bf 8.0 \pm 0.7$ & $92.9 \pm 0.2$ & $7.9 \pm 0.8$  \\
									   & $0.15$ & \underline{$91.3 \pm 0.1$} & \underline{$6.5 \pm 0.9$} & \underline{$89.4 \pm 0.0$} & \underline{$4.8 \pm 0.1$} & \underline{$89.8 \pm 0.1$} & \underline{$5.2 \pm 0.1$} & $\bf 93.1 \pm 0.1$ & $\bf 8.2 \pm 0.6$ & $93.0 \pm 0.2$ & $7.8 \pm 0.8$ \\
									   & $0.20$ & \underline{$91.2 \pm 0.2$} & \underline{$6.6 \pm 0.6$} & \underline{$88.5 \pm 0.1$} & \underline{$4.0 \pm 0.4$} & \underline{$89.3 \pm 0.1$} & \underline{$5.3 \pm 0.4$} & $\bf 93.1 \pm 0.1$ & $\bf 7.9 \pm 0.6$ & $\bf 93.1 \pm 0.1$ & $\bf 8.2 \pm 0.6$ \\
									   & $0.25$ & \underline{$90.9 \pm 0.1$} & \underline{$6.8 \pm 0.8$} & \underline{$87.4 \pm 0.3$} & \underline{$3.6 \pm 0.5$} & \underline{$88.9 \pm 0.1$} & \underline{$5.4 \pm 0.3$} & $92.9 \pm 0.1$ & $7.6 \pm 0.5$ & $\bf 93.0 \pm 0.2$ & $\bf 7.8 \pm 0.7$ \\
		\hline
	\end{tabular}
	}
 \vspace{-4mm}
\end{table*}

\noindent \textbf{More experimental results.} Due to the space limitation, we defer more experimental results on attacking individual fairness on graph neural networks in Appendix~\ref{sec:additional_results_individual_fairness}. More specifically, we present the performance evaluation under different metrics, i.e., Macro F1 and AUC, as well as the effectiveness of \method~with a different victim model, i.e., InFoRM-GNN~\cite{kang2020inform}, which mitigates individual bias.

==> neurips_2023/05related.tex <==
\vspace{-2mm}
\section{Related Work}
\vspace{-2mm}
\noindent \textbf{Algorithmic fairness on graphs} aims to obtain debiased graph learning results such that a pre-defined fairness measure can be satisfied with respect to the nodes/edges in the graph. Several definitions of the fairness has been studied so far. Group fairness in graph embedding can be ensured via several ways, including adversarial learning-based methods~\cite{bose2019compositional, dai2021say}, random walk-based methods~\cite{rahman2019fairwalk, khajehnejad2022crosswalk} and dropout-based methods~\cite{spinelli2021fairdrop}. Individual fairness on graphs can be ensured via Lipschitz regularization~\cite{kang2020inform} and learning-to-rank~\cite{dong2021individual}. Other than the aforementioned two fairness definitions, several other fairness definitions are studied in the context of graph learning, including counterfactual fairness~\cite{agarwal2021towards, ma2021graph}, degree fairness~\cite{tang2020investigating, kang2022rawlsgcn, liu2023generalized}, dyadic fairness~\cite{masrour2020bursting, li2021dyadic} and max-min fairness~\cite{rahmattalabi2019exploring, tsang2019group}. For a comprehensive review of related works, please refer to recent surveys~\cite{zhang2022fairness, choudhary2022survey, dong2022fairness} and tutorials~\cite{kang2021fair, kang2022algorithmic}. It should be noted that our work aims to attack fairness (i.e., making the model more biased) rather than ensuring fairness as in the aforementioned literature.

% In this section, we briefly review related works from the following two perspectives: (1) algorithmic fairness on graphs and (2) adversarial attacks on graphs.

% \noindent \textbf{Algorithmic fairness on graphs} aims to obtain debiased graph learning results such that a pre-defined fairness definition can be satisfied with respect to the nodes/edges in the graph.
% For group fairness,
% Bose et al.~\cite{bose2019compositional} debias node embeddings for a set of sensitive attributes compositionally.
% Rahman et al.~\cite{rahman2019fairwalk} propose FairWalk that assigns an equal probability for each demographic group during the random walk process.
% Dai and Wang~\cite{dai2021say} debias graph neural networks through an adversarial learning framework.
% Spinelli et al.~\cite{spinelli2021fairdrop} find a debiased graph structure by dropping out edges randomly.
% For individual fairness,
% Kang et al.~\cite{kang2020inform} provide the first systematic study for graph learning through Lipschitz regularization,
% which is further extended to a multi-view graph by Wang et al.~\cite{wang2022ifig}.
% Dong et al.~\cite{dong2021individual} propose a ranking-based individual fairness definition to avoid the distance comparison in the Lipschitz continuity-based definition.
% Regarding counterfactual fairness,
% Agarwal et al.~\cite{agarwal2021towards} perturb the sensitive attribute of a node to learn the counterfactually fair node embeddings.
% Ma et al.~\cite{ma2022learning} perturb both the sensitive attribute and the local neighborhood of a node to achieve fairness.
% Other than the aforementioned three fairness definitions, several other fairness definitions are studied in the context of graph learning. For instance,
% % dyadic fairness
% Marsour et al.~\cite{masrour2020bursting} achieve dyadic fairness in link prediction via adversarial learning.
% Li et al.~\cite{li2021dyadic} theoretically study the relationship between dyadic fairness and edge weights.
% % degree fairness
% Tang et al.~\cite{tang2020investigating} achieve degree fairness by learning degree-specific with recurrent neural networks.
% Kang et al.~\cite{kang2022rawlsgcn} ensure degree fairness by normalizing the input graph into a doubly stochastic format.
% % maximin fairness
% Rahmattalabi et al.~\cite{rahmattalabi2019exploring} ensure max-min fairness for robust graph covering problem~\cite{tzoumas2017resilient} by solving mixed integer linear program. 
% For a comprehensive review of related works, please refer to existing surveys~\cite{zhang2022fairness, choudhary2022survey, dong2022fairness} and tutorials~\cite{kang2021fair, kang2022algorithmic}. It should be noted that our work aims to attack fairness (i.e., making the model more biased) rather than ensuring fairness as done by the aforementioned literature.

\noindent \textbf{Adversarial attacks on graphs} aim to exacerbate the utility of graph learning models by perturbing the input graph topology and/or node features. Several approaches have been proposed to attack graph learning models, including reinforcement learning~\cite{dai2018adversarial}, bi-level optimization~\cite{zugner2018adversarial, zugner2019adversarial}, projected gradient descent~\cite{sun2018data, xu2019topology} and edge rewiring/flipping~\cite{bojchevski2019adversarial, ma2021graph}. Other than adversarial attacks that worsen the utility of a graph learning model, a few efforts have been made to attack the fairness of a machine learning model for IID tabular data via label flipping~\cite{mehrabi2021exacerbating}, adversarial data injection~\cite{solans2021poisoning, chhabra2021fairness}, adversarial sampling~\cite{van2022poisoning}. Different from \cite{solans2021poisoning, mehrabi2021exacerbating, chhabra2021fairness, van2022poisoning}, we aim to poison the input graph via structural modifications on the topology rather than injecting adversarial data sample(s). The most related work to our proposed method is by Hussain et al.~\cite{hussain2022adversarial}, which degrade the group fairness of graph neural networks by randomly injecting edges for nodes in different demographic groups and with different class labels. In contrast, our proposed method could attack \textit{any} fairness definition for \textit{any} graph learning models via arbitrary edge manipulation operations, as long as the bias function and the utility loss are differentiable.

% \noindent \textbf{Adversarial attacks on graphs} aim to exacerbate the utility of graph learning models by perturbing the input graph topology and/or node features. For example, 
% % graph neural networks
% Dai et al.~\cite{dai2018adversarial} leverage reinforcement learning for black-box poisoning attacks on graph neural networks.
% Z{\"u}gner et al.~\cite{zugner2018adversarial} attack a nonlinear graph neural network by attacking a surrogate linear graph neural network, as well as maintaining the degree distribution and feature co-occurrence.
% Z{\"u}gner and G{\"u}nnemann~\cite{zugner2019adversarial} select the perturbations using meta-gradient.
% Xu et al.~\cite{xu2019topology} utilize projected gradient descent for untargeted white-box attacks on graph neural networks.
% Ma et al.~\cite{ma2021graph} attack a graph neural network by rewiring edges.
% % graph-based SSL
% Liu et al.~\cite{liu2019unified} attack the graph-based semi-supervised classification and regression tasks via label propagation and manifold regularization.
% % network embedding
% Chen et al.~\cite{chen2018fast} attack network embedding algorithms via the fast gradient sign method.
% Sun et al.~\cite{sun2018data} utilize projected gradient descent to attack network embedding algorithms.
% Bojchevski et al.~\cite{bojchevski2019adversarial} investigate the adversarial vulnerability of random walk-based network embedding by performing edge flips. 
% % community detection
% Li et al.~\cite{li2020adversarial} attack community detection algorithms by generating adversarial graphs using variational auto-encoders.
% Other than adversarial attacks that worsen the utility of a graph learning model, a few efforts have been made to attack the fairness of a machine learning model~\cite{solans2021poisoning, mehrabi2021exacerbating, chhabra2021fairness, van2022poisoning, hussain2022adversarial}. 
% % iid setting
% Solans et al.~\cite{solans2021poisoning} generate poisoned data samples using a gradient-based strategy.
% Mehrabi et al.~\cite{mehrabi2021exacerbating} introduce a heuristic label-flipping strategy and an influence function-based strategy to exacerbate the algorithmic bias on IID data. 
% Chhabra et al.~\cite{chhabra2021fairness} propose a two-step adversarial data injection strategy to attack the $k$-median clustering algorithm.
% Van et al.~\cite{van2022poisoning} introduce three methods (adversarial sampling, adversarial labeling and adversarial feature modification) to attack group fairness.
% Different from \cite{solans2021poisoning, mehrabi2021exacerbating, chhabra2021fairness, van2022poisoning}, we aim to poison the input graph via structural modifications on the topology rather than injecting adversarial data sample(s).
% % gnn
% The most related work to our proposed method is by Hussain et al.~\cite{hussain2022adversarial}, who degrade the group fairness of graph neural networks by randomly injecting edges for nodes in different demographic groups and with different class labels. In contrast, our proposed method could attack \textit{any} fairness definition for \textit{any} graph learning models via edge addition/deletion/flip, as long as the bias function and the utility loss are differentiable.

==> neurips_2023/06conclusion.tex <==
\vspace{-2mm}
\section{Conclusion}
\vspace{-2mm}
We study the problem of fairness attacks on graph learning models, whose goal is to amplify the bias while maintaining the utility on the downstream task. We formally define the problem as a bi-level optimization problem, where the upper-level optimization problem maximizes the bias function with respect to a user-defined fairness definition and the lower-level optimization problem minimizes a task-specific loss function. 
We then propose a meta learning-based framework named \method~to poison the input graph using the meta-gradient of the bias function with respect to the input graph.
% To solve the bi-level optimization problem, we propose a meta learning-based framework named \method~to poison the input graph using the meta-gradient of the bias function with respect to it. 
We instantiate \method~by attacking statistical parity on graph neural networks in a binary node classification problem with binary sensitive attributes. Empirical evaluation demonstrates that \method~is effective (consistently amplifying bias) and deceptive (achieving the highest micro F1 score). %across all settings on all datasets. In the future, we will investigate the capability of \method~in attacking equal opportunity and individual fairness, as well as how to scale up the computation of meta-gradient.

==> neurips_2023/07acknowledgements.tex <==
\begin{acks}
\jian{to add after accepted}
\end{acks}
